Monte Carlo parameter study for Seyfert AGN-starburst composite galaxies NGC1068 and NGC7469

Seyfert-starburst composite galaxies host two promising phenomena of non-thermal high-energy radiation. In this regard the IceCube observation of high-energy neutrinos from the direction of the Seyfert-starburst composite galaxy NGC 1068 is not surprising. More recently, another Seyfert-starburst composite galaxy, NGC 7469, has shown hints for neutrino emission at even higher energies. Theoretical investigations could clarify that their so-called AGN corona is the most-likely origin of these neutrinos due to the need of being partially $\gamma$-ray opaque. In this work, we present an updated version of our Seyfert-starburst composite model from 2022, that accounts for a proper treatment of the stochastic acceleration processes in the AGN corona and the secondary electrons and positrons from leptonic radiation processes. Moreover, we use a Markov Chain Monte Carlo (MCMC) approach to study the parameter space of these two potential high-energy neutrino sources under consideration of the given prior knowledge. In the case of NGC 1068, we can successfully explain its non-thermal observational features, where both its AGN corona and starburst ring are needed to account for the observations at high- energies. In the case of NGC 7469, the high-energy signatures can only be explained assuming a small coronal radius and the including external $\gamma\gamma$-pair attenuation. In general, both sources exhibit a strong influence of the $\gamma$-ray opaqueness on the results, highlighting the need for an accurate treatment of the intrinsic coronal X-ray field and the spatial extent of the $\gamma$-ray production site.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

